Towards Better Meta-Initialization with Task Augmentation for Kindergarten-aged Speech Recognition

Children's automatic speech recognition (ASR) is always difficult due to, in part, the data scarcity problem, especially for kindergarten-aged kids. When data are scarce, the model might overfit to the training data, and hence good starting points for training are essential. Recently, meta-learning was proposed to learn model initialization (MI) for ASR tasks of different languages. This method leads to good performance when the model is adapted to an unseen language. However, MI is vulnerable to overfitting on training tasks (learner overfitting). It is also unknown whether MI generalizes to other low-resource tasks. In this paper, we validate the effectiveness of MI in children's ASR and attempt to alleviate the problem of learner overfitting. To achieve model-agnostic meta-learning (MAML), we regard children's speech at each age as a different task. In terms of learner overfitting, we propose a task-level augmentation method by simulating new ages using frequency warping techniques. Detailed experiments are conducted to show the impact of task augmentation on each age for kindergarten-aged speech. As a result, our approach achieves a relative word error rate (WER) improvement of 51% over the baseline system with no augmentation or initialization.

==> Tables/Table2.tex <==
\begin{table*}[th]
    \caption{Performance of first-order model-agnostic meta-learning (FOMAML) and data augmentation mechanisms in meta-learning using speed perturbation (SP) on different age groups of augmented tasks on the Kindergarten development and test sets. The age groups are added in two ways, either from the most similar age group to the most distinct age group in the forward order, or from the most distinct age group to the most similar age group in the reverse order.}
    \centering
    \begin{tabular}{ccccc}
        \hline
        Exp. & Aug Age Group & \# Total Tasks & Dev & Test \\
        \hline\hline
        0 & - & 9 & 35.21 & 30.68 \\
        \hline
        f1 & G2 & 11 & 36.27 & 30.37 \\
        f2 & G2-G3 & 13 & 34.86 & 30.93 \\
        f3 & G2-G4 & 15 & 35.56 & 29.31 \\
        f4 & G2-G5 & 17 & 34.51 & 29.5 \\
        f5 & G2-G6 & 19 & 33.1 & 28.69 \\
        f6 & G2-G7 & 21 & 33.8 & 28.25 \\
        f7 & G2-G8 & 23 & 34.86 & 27.94 \\
        f8 & G2-G9 & 25 & 34.51 & 29.31 \\
    %    \hline
    %\end{tabular}
    %\begin{tabular}{ccccc}
    %    \hline
    %    Exp. & Aug Age Group & \# Total Tasks & Dev & Test \\
        \hline
        r1 & G10 & 11 & 34.51 & 32.61 \\
        r2 & G10-G9 & 13 & 33.1 & 31.61 \\
        r3 & G10-G8 & 15 & 35.92 & 31.05 \\
        r4 & G10-G7 & 17 & 36.27 & 30.62 \\
        r5 & G10-G6 & 19 & 35.21 & 29.68 \\
        r6 & G10-G5 & 21 & 35.92 & 29.56 \\
        r7 & G10-G4 & 23 & 36.27 & 28.19 \\
        r8 & G10-G3 & 25 & 34.51 & 29.62 \\
        \hline
        9 & all & 27 & 34.86 & 27.5 \\
        \hline
    \end{tabular}
    \label{tab:tab2}
\end{table*}

